Nested replicator dynamics, nested logit choice, and similarity-based learning

We consider a model of learning and evolution in games whose action sets are endowed with a partition-based similarity structure intended to capture exogenous similarities between strategies. In this model, revising agents have a higher probability of comparing their current strategy with other strategies that they deem similar, and they switch to the observed strategy with probability proportional to its payoff excess. Because of this implicit bias toward similar strategies, the resulting dynamics - which we call the nested replicator dynamics - do not satisfy any of the standard monotonicity postulates for imitative game dynamics; nonetheless, we show that they retain the main long-run rationality properties of the replicator dynamics, albeit at quantitatively different rates. We also show that the induced dynamics can be viewed as a stimulus-response model in the spirit of Erev & Roth (1998), with choice probabilities given by the nested logit choice rule of Ben-Akiva (1973) and McFadden (1978). This result generalizes an existing relation between the replicator dynamics and the exponential weights algorithm in online learning, and provides an additional layer of interpretation to our analysis and results.

==> Body/Multiple.tex <==
%----------------------------------------------------------------------
%%% APPENDIX
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


We now proceed to derive and discuss a general version of the revision protocol \eqref{eq:PPI-2} and the induced dynamics \eqref{eq:NRD-single} that allow for multiple layers of similarities between strategies.
As before, our main aim will be to examine how the evolution of the population's aggregate behavior over time is influenced by different degrees of similarity within the agents' revision process.
%Other than certain mathematical subtleties that arise,
%which necessitate somewhat heavier notation, our model is similar in spirit to earlier works considering similarities between strategies, \cf \attn and references therein.
%In this regard,
Because the notation involved can become cumbersome at times, it will help to keep in mind as a running example a group of commuters who regard
different departure times on a given transport route as most similar,
different routes using a given mode of transport as less similar,
and alternatives using distinct modes of transport as the least similar.


%----------------------------------------------------------------------
%%% Generalities
%----------------------------------------------------------------------
\subsection{Multiple layers of similarities: basic notions and definitions}
\label{eq:attributes}

To account for multiple layers of similarities between actions, we will assume that the players' set of strategies comes equipped with a nest of increasingly finer partitions as follows:

\begin{definition}
\label{def:struct}
A \emph{similarity structure} \textendash\ or \emph{hierarchy} \textendash\ on $\pures$ is a tower of nested \emph{similarity partitions} $\classes\atlvl{\lvl}$, $\lvl=0,\dotsc,\nLvls$, of $\pures$ such that
\begin{equation}
\{\pures\}
	\eqdef \classes\atlvl{0}
	\refined \classes\atlvl{1}
	\refined \dotsb
	\refined \classes\atlvl{\nLvls}
	\defeq \setdef{\{\pure\}}{\pure \in \pures}
\end{equation}
where the notation ``$\mathcal{P}\refined \mathcal{Q}$'' means that the partition $\mathcal{Q}$ of $\pures$ is \emph{finer} than $\mathcal{P}$, \ie every element of $\mathcal{Q}$ is a subset of some element of $\mathcal{P}$.%
\footnote{The trivial partition $\classes\atlvl{0} = \{\pures\}$ does not carry any information in itself, but it has been included for completeness and notational convenience later on.
We also assume that $\classes\atlvl{\nLvls}$ completely resolves $\pures$ as, otherwise, any two unresolved elements would be indistinguishable.}
\end{definition}

In this definition, each partition $\classes\atlvl{\lvl}$, $\lvl=0,\dotsc,\nLvls$, captures a succcessively finer attribute of the elements of $\pures$:
for example, in the commuting example,
the coarsest partition $\classes\atlvl{1}$ would correspond to the available modes of transport,
the second partition $\classes\atlvl{2} \refines \classes\atlvl{1}$ to different routes within a given transport mode,
and
$\classes\atlvl{3} \refines \classes\atlvl{2}$ to different times of departure for a given route.
To keep track of all this, each constituent set $\class$ of a partition $\classes\atlvl{\lvl}$ will be referred to as a \emph{similarity class of level $\lvl$}, and we assume it collects all elements of $\pures$ that share a common instance of the attribute defining $\classes\atlvl{\lvl}$ (for example, all metro line combinations going from Montparnasse to Gare de l'Est in Paris).
%for example, a similarity class for the attribute ``artist'' might consist of all Beethoven symphonies, all songs by Led Zeppelin, etc.

More succinctly, a similarity structure on $\pures$ can be represented by the disjoint union
\begin{equation}
\label{eq:struct}
\struct
	\defeq \coprod\nolimits_{\lvl=0}^{\nLvls} \classes\atlvl{\lvl}
	\equiv \union\nolimits_{\lvl=0}^{\nLvls} \setdef{(\set,\lvl)}{\set\in\classes\atlvl{\lvl}}
%	= \setdef{(\set,\lvl)}{\set\in\classes\atlvl{\lvl},\lvl=0,\dotsc,\nLvls}
\end{equation}
of all class/level pairs of the form $(\set,\lvl)$ for $\set\in\classes\atlvl{\lvl}$.
To simplify notation,
%In a slight abuse of terminology,
if there is no danger of confusion,
%the pair $(\class,\lvl)$ will also be referred to as a ``class'',
%and
we will not differentiate between $\class$ and $(\class,\lvl)$;
%we will write $\class\in\classes\atlvl{\lvl}$ and $\pure\in\class$ instead of $\set\in\classes\atlvl{\lvl}$ and $\pure\in\set$ respectively.
by contrast, when we need to unambiguously keep track of the level index $\lvl$ of $\class$, we will write $\lvl = \attof{\class}$.
%distinguish between a class and its underlying set, we will write $\set = \elemof{\class}$ for the set of alternatives contained in $\class$ and
%$\lvl = \attof{\class}$ for the attached attribute label.
%
%\smallskip
%%\setcounter{remark}{0}
%\begin{remark*}
The reason for including the attribute index $\lvl$ in the definition of a similarity class is that a set of alternatives may appear in distinct partitions of $\pures$ in a different context.
For example, in Paris, the only (reasonable) way to go from Denfert Rochereau to Place d'Italie via metro is to take Line 6;
in this case, the timetable of Line 6 simultaneously represents the set of ``all ways of going from Denfert Rochereau to Place d'Italie via metro'' (a tier $1$ similarity class in our running example), as well as the set of ``all ways of going from Denfert Rochereau to Place d'Italie via Line 6'' (a tier $2$ class).
%if ``IV'' is the only album by Led Zeppelin in a music catalogue, the album's track list represents both the set of ``all songs in IV'' as well as the set of ``all Led Zeppelin songs'' in the catalogue in question.
In other words, the attribute of interest is different in each case \textendash\ ``transport mode'' in the former versus ``line combination'' in the latter \textendash\ and this additional information would be lost in the non-discriminating union $\union_{\lvl=0}^{\nLvls} \classes\atlvl{\lvl}$.
%\endenv
%\end{remark*}

Moving forward, if a class $\parent\in\classes\atlvl{\lvl}$ contains the class $\child\in\classes\atlvl{\lvlalt}$ for some $\lvlalt>\lvl$, we will say that $\child$ is a \emph{descendant} of $\parent$ and we will write ``$\child \desc \parent$'' (resp.``$\parent \anc \child$'' when $\parent$ is an \emph{ancestor} of $\child$).%
\footnote{The corresponding weak relation ``$\desceq$'' (resp.~``$\anceq$'') is defined in the standard way, \ie allowing for the case $\attof{\child} = \attof{\parent}$ which in turn implies that $\child = \parent$.
Clearly, the relation ``$\desc$'' defines a strict partial order on $\struct$, so $\struct$ may be seen as a poset in its own right.}
As a special case of this relation, if $\child \desc \parent$ and $\lvlalt = \lvl+1$, we will say that $\child$ is a \emph{child} of $\parent$ and we will write ``$\child \childof \parent$'' (resp.~$\parent$ is a \emph{parent} of $\child$ when $\parent \parentof \child$).
%Any two children of the same parent class will be called \emph{siblings}, and we will write ``$\sibling$'' for the corresponding relation.
More generally, when we wish to focus on descendants sharing a certain attribute, we will write ``$\child \desceq[\lvl] \parent$'' as shorthand for the predicate ``$\child \desceq \parent$ and $\attof{\child} = \lvl$''.
In a similar vein, given an arbitrary class $\class\in\struct$, we will write $\classof[\lvl]{\class}$ for the $\lvl$-th type ancestor of $\class$, \ie the (necessarily unique) similarity class $\class\atlvl{\lvl}\in\classes\atlvl{\lvl}$ containing $\class$ (obviously, we assume here that $\attof{\class} \geq \lvl$).
%some arbitrary class $\class\in\classes$ with $\attof{\class} \geq \lvl$,
Finally, we will say that two classes $\class,\classalt\in\pures$ are \emph{similar with respect to attribute $\classes\atlvl{\lvl}$} if and only if $\classof[\lvl]{\class} = \classof[\lvl]{\classalt}$, in which case we will write $\class \sibling[\lvl] \classalt$.%
\footnote{The notations $\classof{\pure}$ and $\pure\sibling\purealt$ will be reserved for elements of $\pures$ and immediate similarities respectively (\ie when $\lvl = \nLvls-1$).}


Building on the above, a similarity structure on $\pures$ can also be represented graphically as a rooted directed tree \textendash\ or \emph{arborescence} \textendash\ by connecting two classes $\parent,\child\in\struct$ with a directed edge $\parent\to\child$ whenever $\parent \parentof \child$ (\cf \cref{fig:tree} above).
By construction, the root of this tree is $\source$ itself,%
\footnote{Stricto sensu, the root of the tree is $(\pures,0)$, but since there is no danger of confusion, the attribute label ``0'' will be dropped in this case.}
and
the unique directed path $\source \equiv \class\atlvl{0} \parentof \class\atlvl{1} \parentof \dotsb \parentof \class\atlvl{\lvl} \equiv \class$ from $\source$ to any class $\class\in\struct$ will be referred to as the \emph{lineage} of $\class$.
For notational simplicity, we will not distinguish between $\struct$ and its graphical representation, and we will use the two interchangeably.


%----------------------------------------------------------------------
%% Class figure begins here

\begin{figure}[tbp]
\ctikzfig{Figures/tree1}
\caption{Graphical representation of a $3$-tier similarity structure as a rooted tree.}
\label{fig:tree}
\end{figure}

%% Class figure ends here
%----------------------------------------------------------------------


%----------------------------------------------------------------------
%%% Revision protocols
%----------------------------------------------------------------------
\subsection{\Acl{PPI} and the \acl{NRD}}
\label{sec:SPPI}

With all this in hand, we are finally in a position to adapt the notion of \acl{PPI} in the presence of a similarity structure $\classes\atlvl{0} \refined \classes\atlvl{1} \refined \dotsb \refined \classes\atlvl{\nLvls}$ as above.
Working as in \cref{sec:single}, we will consider a multi-stage revision protocol that unfolds as follows:
\begin{enumerate}
\item
When a revision opportunity arises, the revising agent first decides which attribute to focus on (mode of transport, route, departure time, etc.).
Formally, this amounts to choosing a similarity tier $\lolvl \in \lolvls$:
with probability $\rate\atlvl{0}$, the agent does not take into account any similarities whatsoever;
with probability $\rate\atlvl{1}$, the agent considers the pool of strategies that are similar to their own up to tier $1$ (\eg they employ the same mode of transport but may switch routes or departure times);
with probability $\rate\atlvl{2}$, they consider those strategies that are similar to their own up to tier $2$ (\eg they take the same route with the same mode of transport, but may consider switching departure times);
and so on through the entire hierarchy of similarities.%
\footnote{Our analysis can be extended to allow each similarity class $\class\in\struct$ to have its individual revision rate $\rate\atlvl{\class}$.
This extension is significantly more cumbersome in terms of notation, but is otherwise straightforward.}

\item
Conditioned on the choice of tier $\lolvl\in\lolvls$, the revising agent meets another individual drawn uniformly at random from the sub-population of agents playing a strategy from the corresponding similarity class $\class\atlvl{\lolvl}$.
Thus, if the population is at state $\strat\in\strats$, the probability that a revising $\pure$-strategist encounters a $\purealt$-strategist is
\begin{align}
\label{eq:meet-single}
\pdist_{\pure\purealt}
	= \rate\atlvl{0} \, \strat_{\purealt}
		+ \rate\atlvl{1} \strat_{\purealt} \frac{\oneof{\purealt\sibling[1]\pure}}{\sum_{\alt\pure\sibling[1]\pure} \strat_{\alt\pure}}
		\dotsb
		+ \rate\atlvl{\nLvls-1} \strat_{\purealt} \frac{\oneof{\purealt\sibling[\nLvls-1]\pure}}{\sum_{\alt\pure\sibling[\nLvls-1]\pure} \strat_{\alt\pure}}
%	\notag\\
	= \sum_{\lolvl=0}^{\nLvls-1} \rate\atlvl{\lolvl} \strat_{\purealt \given \classof[\lolvl]{\pure}}
\end{align}
where, as discussed above,
\begin{equation}
\label{eq:classof}
\classof[\lolvl]{\pure}
	= \setdef{\class\atlvl{\lolvl}\in\classes\atlvl{\lolvl}}{\class\atlvl{\lolvl}\ni\pure}
\end{equation}
denotes the ancestor of $\pure$ in $\classes\atlvl{\lolvl}$ (that is, the strategies of $\pures$ that are similar to $\pure$ at level $\lolvl$) while, as per \eqref{eq:strat-cond}, the notation
\begin{equation}
\label{eq:strat-cond-multi}
\strat_{\purealt \given \classof[\lolvl]{\pure}}
	= \oneof{\purealt \sibling[\lolvl] \pure} \frac{\strat_{\purealt}}{\strat_{\classof[\lolvl]{\pure}}}
\end{equation}
stands for the relative frequency of $\purealt$-strategists within the sub-population of $\classof[\lolvl]{\pure}$-type strategists (\ie the part of the population playing a strategy similar to $\pure$ at level $\lolvl$).

\item
Finally, as in the case of \eqref{eq:PPI}, the revising agent observes the comparator's payoff:
if it is higher, they imitate the comparator with probability proportional to the observed payoff difference;
otherwise, the revising agent skips the opportunity to switch.
\end{enumerate}

Thus, putting everything together, we obtain the \acli{NPPI} protocol
%Expanding on the ideas presented in \cref{sec:single}, conditional switch rates under the $\nLvls$-level analogue of \acl{PPI} are given by
\begin{equation}
\label{eq:NPPI}
\tag{NPPI}
\switch_{\pure\purealt}(\py,\strat)
	= \sum_{\lolvl=0}^{\nLvls-1}
		\rate\atlvl{\lolvl}\,
		\strat_{\purealt \given \classof[\lolvl]{\pure}}
		\pospart{\py_{\purealt} - \py_{\pure}},
\end{equation}
where the ``intra-layer'' testing probabilities $\rate\atlvl{\lolvl} \geq 0$ satisfy
\begin{equation}
\label{eq:normal}
\sum_{\lolvl=0}^{\nLvls-1} \rate\atlvl{\lolvl}
%\rate\atlvl{0} + \rate\atlvl{1} + \dotsb + \rate\atlvl{\nLvls}
	= 1.
\end{equation}
%to avoid trivialities, we assume that the revision rates $\rate\atlvl{\lolvl}$ are nonnegative for $\lolvl\in\{1,\dotsc,\nLvls-1\}$, and positive for $\lolvl=0$.
%We also recall that the case $\lolvl=\nLvls$ is meaningless in terms of switches, as the only possible switch would be from $\pure$ to itself;
%however, for completeness, we also introduce the trivial $\nLvls$-level switch rate $\rate\atlvl{\nLvls} = 0$.
%Finally, to facilitate comparisons and streamline our presentation, we will again make the normalization assumption
%\begin{equation}
%\label{eq:normal}
%%\sum_{\lolvl=0}^{\nLvls} \rate\atlvl{\lolvl}
%\rate\atlvl{0} + \rate\atlvl{1} + \dotsb + \rate\atlvl{\nLvls}
%	= 1.
%\end{equation}
Under this layered version of pairwise proportional imitation, a revising agent effectively runs $\nLvls$ revision procedures simultaneously.
In the $\lolvl$-th level procedure, which runs at rate $\rate\atlvl{\lolvl}$ and concerns the $\lolvl$-th attribute $\classes\atlvl{\lolvl}$ of $\struct$, the agent considers switches from their current strategy $\pure$ to alternatives $\purealt\in\classof[\lolvl]{\pure}$ that are similar to $\pure$ at level $\lolvl$ (the case $\lolvl=0$ corresponds to switches that disregard any exogenous similarities while the case $\lolvl=\nLvls$ is ignored as the only possible switch would be from $\pure$ to $\pure$).
%In more detail, this means that the revising agent first observes the action of a randomly selected individual playing an action in $\classof[\lolvl]{\pure}$, so the (conditional) probability of observing $\purealt\in\pures$ is equal to the relative population share $\strat_{\purealt \given \classof[\lolvl]{\pure}} = \strat_{\purealt} / \strat_{\classof[\lolvl]{\pure}}$.
Next, the agent switches to action $\purealt$ only if the payoff to $\purealt$ is higher than that of $\pure$, and then with probability proportional to the payoff difference $\pospart{\py_{\purealt} - \py_{\pure}}$.
In this way, the nested protocol \eqref{eq:NPPI} incorporates the various tiers of exogenous similarity induced by the structure $\struct$ and assumes that \emph{all} degrees of similarity are examined concurrently (though possibly at different rates).

Now, to derive the dynamics on $\strats$ induced by \eqref{eq:NPPI}, a direct substitution into \eqref{eq:MD} yields
\begin{align}
\dot\strat_{\pure}
	&= \sum_{\lolvl=0}^{\nLvls-1}
		\rate\atlvl{\lolvl} \strat_{\pure}
		\bracks*{
			\sum_{\purealt\in\pures}
				\strat_{\purealt\given\classof[\lolvl]{\pure}}
				\pospart{\payv_{\pure}(\strat) - \payv_{\purealt}(\strat)}
			- \sum_{\purealt\in\pures}
				\strat_{\purealt\given\classof[\lolvl]{\pure}}
				\pospart{\payv_{\purealt}(\strat) - \payv_{\pure}(\strat)}
		} % end bracks
\end{align}
and hence, recalling the definition \eqref{eq:pay-class} of mean class payoffs $\classpay_{\class}(\strat) = \sum_{\pure\in\class} \strat_{\pure \given \class} \payv_{\pure}(\strat)$ and rearranging, we obtain the ($\nLvls$-\emph{level}) \acli{NRD}
\begin{equation}
\label{eq:NRD}
\tag{NRD}
\dot \strat_{\pure}
	= \strat_{\pure}
		\sum_{\lolvl=0}^{\nLvls-1}
		\rate\atlvl{\lolvl}\,
		\bracks{\payv_{\pure}(\strat) - \classpay_{\classof[\lolvl]{\pure}}(\strat)}.
\end{equation}
These dynamics will be our main focus in the sequel, so some remarks are in order.

First, as can already be seen from the definition of the nested protocol \eqref{eq:NPPI}, the original replicator system \eqref{eq:RD} is recovered immediately for $\rate\atlvl{0}=1$ and $\rate\atlvl{1} = \dotsb = \rate\atlvl{\nLvls-1} = 0$.
In this case, revising agents pay no heed to any exogenous similarities when selecting a comparator, so it stands to reason that the induced dynamics boil down to \eqref{eq:RD}.
Otherwise, in the general case, the per capita growth rate of a strategy $\pure\in\pures$ under \eqref{eq:NRD} is a convex combination of payoff differences between $\payv_{\pure}(\strat)$ and the subpopulation means $\classpay_{\classof[\lolvl]{\pure}}(\strat)$ evaluated at all levels of resemblance to $\pure$ \textendash\ from the maximum possible degree (when $\lolvl=\nLvls-1$) to no similarities whatsoever when $\lolvl=0$.

A second observation is that, by summing \eqref{eq:NRD} over all alternatives comprising a given similarity class $\class\in\classes\atlvl{\lvl}$, we obtain the class dynamics
%changes in the population share of each similarity class $\class$ under \eqref{eq:NRD} can be described by the class dynamics
\begin{equation}
\label{eq:NRD-class}
\dot\strat_{\class}
	= \sum_{\pure\in\class} \dot\strat_{\pure}
	= \strat_{\class}
		\sum_{\lolvl=0}^{\lvl-1}
		\rate\atlvl{\lolvl}\,
		\bracks{\classpay_{\class}(\strat) - \classpay_{\classof[\lolvl]{\class}}(\strat)}
\end{equation}
where, as usual, $\classof[\lolvl]{\class}$ denotes the $\lolvl$-th level ancestor of $\class$.
These dynamics are formally analogous to \eqref{eq:NRD} with $\lvl$ levels of nesting instead of $\nLvls$, and with a coarser similarity hierarchy that does not differentiate actions beyond their $\lvl$-th attribute.
%finely than the $\lvlalt$-th level classes.
However, as in \eqref{eq:NRD-single-class}, the average payoffs $\classpay_{\class}(\strat)$ and $\classpay_{\classof[\lolvl]{\pure}}(\strat)$ appearing in \eqref{eq:NRD-class} depend not only on the aggregate population shares $\strat_{\class}$, but on the \emph{complete} population state $\strat \in \strats$, so \eqref{eq:NRD-class} is not an autonomous system in this regard.

Finally, as in the case of \eqref{eq:PPI-2}, it is worth noting that imitation rates under \eqref{eq:NPPI} are always higher between similar strategies compared to dissimilar strategies, and the higher the degree of similarity, the higher the imitation rate.
Indeed, by \eqref{eq:strat-cond-multi}, the agents' conditional imitation rates under \eqref{eq:NPPI} are
\begin{equation}
\label{eq:imit-multi}
\imit_{\pure\purealt}(\py,\strat)
	= \frac{\switch_{\pure\purealt}(\py,\strat)}{\strat_{\purealt}}
	= \sum_{\lolvl=0}^{\nLvls-1}
		\rate\atlvl{\lolvl}\,
		\frac{\oneof{\purealt \sibling[\lolvl] \pure}}{\strat_{\classof[\lolvl]{\pure}}}
		\cdot
		\pospart{\py_{\purealt} - \py_{\pure}}
	= \pospart{\py_{\purealt} - \py_{\pure}}
		\cdot \!\!\sum_{\lolvl=0}^{\deg(\pure,\purealt)}\!\!
			\frac{\rate\atlvl{\lolvl}}{\strat_{\classof[\lolvl]{\pure}}}
\end{equation}
where $\deg(\pure,\purealt) \defeq \max\setdef{\lolvl=0,\dotsc,\nLvls-1}{\pure \sibling[\lolvl] \purealt}$ denotes the maximum degree of similarity between $\pure$ and $\purealt$, \ie the finest attribute that they share.
%Consequently, for a given value of the payoff differential $\pospart{\py_{\purealt} - \py_{\pure}}$,
%if two strategies $\pure,\purealt\in\pures$ have the same payoff differential, say $\pospart{\py_{\purealt} - \py_{\pure}} = 1$,
Thus, all other things being equal, the imitation rate of $\purealt$-strategists by $\pure$-strategists is highest when $\pure$ and $\purealt$ are most similar (\eg different train departure times on a given transport route for the same medium), and lowest when $\pure$ and $\purealt$ are least similar (\eg different transport modes altogether).

As in the case of \eqref{eq:PPI-2}, this increased affinity toward similar strategies is an \emph{intrinsic} feature of the agents' revision mechanism, and is not enforced extrinsically \textendash\ \ie by maintaining the same encounter probabilities for the entire population but increasing the probability of imitating more similar strategies.
We discuss this issue in \cref{sec:discussion}.


%----------------------------------------------------------------------
%%% First results
%----------------------------------------------------------------------
\subsection{Rationality properties of the \acl{NRD}}
\label{sec:results}

We are now in a position to state our main result for the long-run behavior of the dynamics \eqref{eq:NRD}, extending the intermediate results presented in \cref{thm:NRD-single} for the single-tier case.
%(which contain \cref{thm:NRD-single} as a special case):
%which shows that the properties of \eqref{eq:NRD-single} stated in \cref{thm:NRD-single} also hold for \eqref{eq:NRD}:

\begin{theorem}
\label{thm:NRD}
Let $\game\equiv\gamefull$ be a population game, let $\struct$ be a similarity hierarchy on $\pures$, and let $\orbit{\time}$ be an interior solution trajectory of the \acl{NRD} \eqref{eq:NRD} for $\game$.
Then:
\begin{enumerate}
[label={\arabic*.},ref=\arabic*]
%\renewcommand{\labelenumi}{\theenumi}

\item
\label[part]{part:dom}
If $\pure \in \pures$ is strictly dominated, then $\lim_{\time\to\infty} \orbit[\pure]{\time} = 0$.

\item
\label[part]{part:stat}
A state $\eq\in\strats$ is stationary if and only if it is a \acl{RE} of $\game$.

\item
\label[part]{part:limit}
If $\orbit{\time}$ converges to $\eq$ as $\time\to\infty$, then $\eq$ is a \acl{NE} of $\game$.

\item
\label[part]{part:Lyap}
If $\eq\in\strats$ is Lyapunov stable, then it is a \acl{NE} of $\game$.

\item
\label[part]{part:ESS}
If $\eq$ is an \ac{ESS} of $\game$, it is asymptotically stable. %\textpar{so it attracts all nearby initial conditions $x(0)\in\strats$}.
In particular, if $\eq$ is a \ac{GESS} of $\game$, it attracts all initial conditions with $\supp(\strat(\tstart)) \supseteq \supp(\eq)$.

\item
\label[part]{part:pot}
If $\game$ is a potential game with potential function $\pot$, then $\pot(\orbit{\time})$ is nondecreasing and $\orbit{\time}$ converges to a connected set of restricted equilibria of $\game$.

\item
\label[part]{part:mon}
If $\game$ is strictly monotone, its \textpar{necessarily unique} \acl{NE} attracts almost all initial conditions \textendash\ and, in particular, all initial conditions with full support.

\end{enumerate}
\end{theorem}

Before discussing the proof of \cref{thm:NRD}, it is worth noting that the dynamics \eqref{eq:NRD} can also be shown to enjoy the following long-term properties:
\begin{enumerate}%
%[\upshape(\itshape i\hspace*{1pt}\upshape)]
\item
Mixed strategies that are iteratively dominated by (possibly) mixed strategies become extinct under \eqref{eq:NRD}.
\item
States that are neutrally stable in the sense of \citet{May82} are also Lyapunov stable.
\item
Asymptotically stable states are perfect \aclp{NE} \citep[in the sense of][]{Sel75}.
%\item
%\acs{ES}* sets \citep{Wei95} are asymptotically stable.
%\item
%If $\eq$ is a \acl{NE} of a null-monotone game,%
%\footnote{A game is null-monotone \textendash\ or \emph{conservative} \textendash\ if \eqref{eq:monotone} holds as an equality for all $\strat,\stratalt \in \strats$.
%For example, $\game$ is conservative if $\payv(\strat) = \mat\strat$ and $\mat$ is symmetric zero-sum \textpar{$\mat = -\mat^{\top}$}.}
%then $\breg_{\nLvls}(\eq,\orbit{\time})$ is a constant of motion.
\item
In random matching games (as per \cref{ex:matching}), the time averages of solution orbits contained in a compact subset of $\relint(\strats)$ converge to the game's set of \aclp{NE}.
\end{enumerate}
To keep our presentation as concise as possible, we omit careful statements and proofs of these additional results, and we focus instead on the properties identified in \cref{thm:NRD}.

The first thing to note here is that, as in the two-level case, the dynamics \eqref{eq:NRD} are \emph{not} payoff-monotonic, so it is fairly surprising to see that they satisfy a range of properties that have long been associated with payoff monotonicity (such as the elimination of strictly dominated strategies and the stability properties of \aclp{NE}).
Expanding on the discussion of \cref{sec:single}, the enabling machinery for these properties of \eqref{eq:NRD} requires a fair degree of hindsight, and is based on the \emph{nested \acl{KL} divergence}
\begin{equation}
\label{eq:NKL}
\tag{NKL}
\breg_{\nLvls}(\base,\strat)
	= \sum_{\lvl=1}^{\nLvls} \diff\atlvl{\lvl}
		\sum_{\class\in\classes\atlvl{\lvl}}
		\base_{\class} \log\frac{\base_{\class}}{\strat_{\class}}.
\end{equation}
where the weights $\diff\atlvl{\lvl}$, $\lvl=1,\dotsc,\nLvls$, are given by the somewhat mysterious expression
\begin{equation}
\label{eq:rate2diff}
\diff\atlvl{\lvl}
	= \begin{cases}
		\rate\atlvl{\lvl} / (\sumrate\atlvl{\lvl-1} \sumrate\atlvl{\lvl})
			&\quad
			\text{if $\lvl=1,\dotsc,\nLvls-1$},
		\\[\smallskipamount]
		1
			&\quad
			\text{if $\lvl=\nLvls$},
	\end{cases}
\end{equation}
with $\sumrate\atlvl{\lvl} = \rate\atlvl{0} + \dotsb + \rate\atlvl{\lvl}$ denoting the total revision rate for attributes of tier $\lvl$ and below (recall here our normalization assumption $\sumrate\atlvl{\nLvls-1} = \rate\atlvl{0} + \dotsb + \rate\atlvl{\nLvls-1} = 1$).

%Just like its one- and two-level counterparts, $\breg_{\nLvls}(\base,\strat)$ provides an asymmetric measure of the ``distance'' of state $\strat$ from state $\base$ that is nonnegative, vanishes only when $\base=\strat$, and blows up to infinity only when $\supp(\base)\nsubseteq\supp(\strat)$.
Intuitively, $\breg_{\nLvls}$ can be viewed as an affine combination of the ordinary \ac{KL} divergence between $\base$ and $\strat$ at different degrees of similarity:
in particular, the $\lvl$-th level terms in \eqref{eq:NKL} add up to the standard \ac{KL} divergence between the class state variables $(\base_{\class\atlvl{\lvl}})_{\class\atlvl{\lvl}\in\classes\atlvl{\lvl}}$ and $(\strat_{\class\atlvl{\lvl}})_{\class\atlvl{\lvl}\in\classes\atlvl{\lvl}}$ in $\simplex(\classes\atlvl{\lvl})$.
As for the \textendash\ admittedly opaque \textendash\ choice of weights $\diff\atlvl{\lvlalt}$ in the definition of $\breg_{\nLvls}$, the specific assignment \eqref{eq:rate2diff} has been meticulously computed to provide the following fundamental link between the nested divergence \eqref{eq:NKL} and the nested dynamics \eqref{eq:NRD}:

\begin{proposition}
\label{prop:KL}
Fix a state $\base\in\strats$ and let $\orbit{\time}$ be an interior solution of \eqref{eq:NRD}.
Then:
\begin{equation}
\label{eq:dKL}
\frac{d}{dt} \breg_{\nLvls}(\base,\orbit{\time})
	= \braket{\payv(\orbit{\time})}{\orbit{\time} - \base}
%	= \pay(\orbit{\time}) - \sum_{\pure\in\pures} \base_{\pure} \payv_{\pure}(\orbit{\time}).
	= \sum_{\pure\in\pures} \payv_{\pure}(\orbit{\time}) \, \parens{\orbit[\pure]{\time} - \base_{\pure}}
\end{equation}
\end{proposition}

In words, \cref{prop:KL} states that, under \eqref{eq:NRD}, the rate of change of the nested \ac{KL} divergence \eqref{eq:NKL} relative to a base point $\base\in\strats$ is the difference between the population average payoff $\pay(\strat) = \braket{\payv(\strat)}{\strat}$ and the average payoff $\braket{\payv(\strat)}{\base}$ of a group of mutants with actions distributed according to $\base$.
The key property highlighted by this interpretation is that two similarity-dependent objects \textendash\ the nested dynamics \eqref{eq:NRD} and the nested \ac{KL} divergence \eqref{eq:NKL} \textendash\ give rise to an invariant quantity that only depends on the game and the population states involved, and is otherwise oblivious of the similarity hierarchy $\struct$.

The key element of the proof of \cref{prop:KL} is that, under the specific weight assignment \eqref{eq:rate2diff}, the time derivative of the nested divergence $\breg_{\nLvls}$ becomes a telescoping sum, with only the finest ($\lvl=\nLvls$) and coarsest ($\lvl=0$) levels surviving in the \acl{RHS} of \eqref{eq:dKL}.
This requires some delicate algebraic manipulations, which we detail below:

\begin{proof}
[Proof of \cref{prop:KL}]
By the definition of the nested \ac{KL} divergence, we have
\begin{equation}
\label{eq:dKL-1}
\frac{d}{dt} \breg_{\nLvls}(\base,\orbit{\time})
	= -\sum_{\lvl=1}^{\nLvls}
		\diff\atlvl{\lvl}\,
		\sum_{\class\in\classes\atlvl{\lvl}} \base_{\class} \frac{\dot \strat_{\class}}{\strat_{\class}}.
\end{equation}
Thus, by substituting the class dynamics \eqref{eq:NRD-class} into \eqref{eq:dKL-1} and rearranging, we get
\begin{align}
\label{eq:dKL-2}
\frac{d}{dt} \breg_{\nLvls}(\base,\orbit{\time})
	&= - \sum_{\lvl=1}^{\nLvls}
		\diff\atlvl{\lvl}
		\sum_{\class\in\classes\atlvl{\lvl}}
			\base_{\class}
			\sum_{\lolvl=0}^{\lvl-1}
				\rate\atlvl{\lolvl}\,
				\bracks{\classpay_{\class}(\strat) - \classpay_{\classof[\lolvl]{\class}}(\strat)}
	\notag\\
	&= \sum_{\lvl=1}^{\nLvls}
		\diff\atlvl{\lvl}
		\sum_{\lolvl=0}^{\lvl-1}
			\rate\atlvl{\lolvl}
			\sum_{\class\in\classes\atlvl{\lvl}}
				\base_{\class}
				\bracks{\classpay_{\class}(\strat) - \classpay_{\classof[\lolvl]{\class}}(\strat)}.
\end{align}
To proceed, note that, for all $\lolvl \leq \lvl$, we have
\begin{align}
\sum_{\class\in\classes\atlvl{\lvl}}
	\base_{\class} \classpay_{\classof[\lolvl]{\class}}(\strat)
	&= \sum_{\class\atlvl{\lolvl} \in \classes\atlvl{\lolvl}}
		\sum_{\class \desceq[\lvl] \class\atlvl{\lolvl}}
			\base_{\class} \classpay_{\classof[\lolvl]{\class}}(\strat)
	\notag\\
	&= \sum_{\class\atlvl{\lolvl} \in \classes\atlvl{\lolvl}}
		\classpay_{\class\atlvl{\lolvl}}(\strat)
		\sum_{\class \desceq[\lvl] \class\atlvl{\lolvl}} \base_{\class}
	= \sum_{\class\atlvl{\lolvl} \in \classes\atlvl{\lolvl}}
		\classpay_{\class\atlvl{\lolvl}}(\strat)\,
		\base_{\class\atlvl{\lolvl}}
	= \braket{\payv(\strat)}{\base}_{\lolvl}
\end{align}
where the notation $\braket{\payv(\strat)}{\base}_{\lolvl}$ stands for
\begin{equation}
\label{eq:classprod}
\braket{\payv(\strat)}{\base}_{\lolvl}
	\defeq \sum_{\class\atlvl{\lolvl}\in\classes\atlvl{\lolvl}} \base_{\class\atlvl{\lolvl}} \classpay_{\class\atlvl{\lolvl}}(\strat)
	\quad
	\text{for all $\base,\strat\in\strats$ and all $\lolvl=0,\dotsc,\nLvls$},
\end{equation}
and
we used the facts that
$\union\setdef{\class}{\class\desceq[\lvl]\class\atlvl{\lolvl}} = \class\atlvl{\lolvl}$
and
$\intersect\setdef{\class}{\class\desceq[\lvl]\class\atlvl{\lolvl}} = \varnothing$ whenever $\lolvl \leq \lvl$.
In this way, \eqref{eq:dKL-2} can be unpacked one attribute at a time to yield
\begin{align}
\label{eq:dKL-3}
%\frac{d}{dt} \breg_{\nLvls}(\base,\orbit{\time})
\eqref{eq:dKL-2}
	&= \sum_{\lvl=1}^{\nLvls}
		\diff\atlvl{\lvl}
		\sum_{\lolvl=0}^{\lvl-1}
			\rate\atlvl{\lolvl}\,
			\bracks{\braket{\payv(\strat)}{\base}_{\lvl} - \braket{\payv(\strat)}{\base}_{\lolvl}}
	\notag\\
	&= \diff\atlvl{1} \rate\atlvl{0} \braket{\payv(\strat)}{\base}_{0}
		- \diff\atlvl{1} \rate\atlvl{0} \braket{\payv(\strat)}{\base}_{1}
	\notag\\
	&+ \diff\atlvl{2} \bracks{\rate\atlvl{0} \braket{\payv(\strat)}{\base}_{0} + \rate\atlvl{1} \braket{\payv(\strat)}{\base}_{1}}
%	\notag\\
%	&\qquad
		- \diff\atlvl{2} \parens{\rate\atlvl{0} + \rate\atlvl{1}}
		\, \braket{\payv(\strat)}{\base}_{2}
	\notag\\
	&\;\:\vdots
	\notag\\
	&+ \diff\atlvl{\nLvls}
		\bracks{\rate\atlvl{0} \braket{\payv(\strat)}{\base}_{0} + \dotsb + \rate\atlvl{\nLvls-1}
		\braket{\payv(\strat)}{\base}_{\nLvls-1}}
%	\notag\\
%	&\hspace{12em}
	- \diff\atlvl{\nLvls}
		\parens{\rate\atlvl{0} + \dotsb + \rate\atlvl{\nLvls-1}}
		\, \braket{\payv(\strat)}{\base}_{\nLvls}
\end{align}
and hence, regrouping all same-level payoff terms, we obtain:
\begin{align}
\label{eq:dKL-4}
\frac{d}{dt} \breg_{\nLvls}(\base,\orbit{\time})
	&= \rate\atlvl{0}
		\parens{\diff\atlvl{1} + \dotsb + \diff\atlvl{\nLvls}}
		\cdot \braket{\payv(\strat)}{\base}_{0}
	\notag\\
	&\;\:\vdots
	\notag\\
	&+ \bracks{\rate\atlvl{\lolvl} \parens{\diff\atlvl{\lolvl+1} + \dotsb + \diff\atlvl{\nLvls}}
		- \diff\atlvl{\lolvl} \parens{\rate\atlvl{0} + \dotsb + \rate\atlvl{\lolvl-1}}}
		\cdot \braket{\payv(\strat)}{\base}_{\lolvl}
	\notag\\
	&\;\:\vdots
	\notag\\
	&- \diff\atlvl{\nLvls}
		\parens{\rate\atlvl{0} + \dotsb + \rate\atlvl{\nLvls-1}}
		\cdot \braket{\payv(\strat)}{\base}_{\nLvls}
	\notag\\
	&= \sum_{\lolvl=0}^{\nLvls}
		\bracks*{\rate\atlvl{\lolvl} \sum_{\lvl=\lolvl+1}^{\nLvls} \diff\atlvl{\lvl}
			- \diff\atlvl{\lolvl} \sum_{\lvl=0}^{\lolvl-1} \rate\atlvl{\lvl}}
		\, \braket{\payv(\strat)}{\base}_{\lolvl}
\end{align}
where, in the last line, we used the empty sum convention $\sum_{j\in\varnothing} \alpha_{j} = 0$.

To proceed, we claim that
\begin{equation}
\label{eq:sumweight}
\diff\atlvl{\lolvl+1} + \dotsb + \diff\atlvl{\nLvls}
	= \frac{1}{\rate\atlvl{0} + \dotsb + \rate\atlvl{\lolvl}}
	= \frac{1}{\sumrate\atlvl{\lolvl}}
	\quad
	\text{for all $\lolvl = 0,\dotsc,\nLvls-1$}.
\end{equation}
Indeed, for $\lolvl=\nLvls-1$, we recover the definition \eqref{eq:rate2diff} of $\diff\atlvl{\nLvls}$.
Otherwise, assume inductively that \eqref{eq:sumweight} holds for some $\lolvl < \nLvls-1$;
then, by \eqref{eq:rate2diff}, we get
\begin{equation}
\label{eq:sumweight-induction}
\diff\atlvl{\lolvl} + \diff\atlvl{\lolvl+1} + \dotsb + \diff\atlvl{\nLvls}
	= \frac{\rate\atlvl{\lolvl}}{\sumrate\atlvl{\lolvl}\sumrate\atlvl{\lolvl-1}}
		+ \frac{1}{\sumrate\atlvl{\lolvl}}
	= \frac{\rate\atlvl{\lolvl} + \sumrate\atlvl{\lolvl-1}}{\sumrate\atlvl{\lolvl}\sumrate\atlvl{\lolvl-1}}
	= \frac{\sumrate\atlvl{\lolvl}}{\sumrate\atlvl{\lolvl}\sumrate\atlvl{\lolvl-1}}
	= \frac{1}{\sumrate\atlvl{\lolvl-1}},
\end{equation}
which completes the inductive step and proves our claim.
Hence, combining \eqref{eq:sumweight} with \eqref{eq:rate2diff}, we get
\begin{equation}
\label{eq:weightrate}
\rate\atlvl{\lolvl} \parens{\diff\atlvl{\lolvl+1} + \dotsb + \diff\atlvl{\nLvls}}
	= \frac{\rate\atlvl{\lolvl}}{\sumrate\atlvl{\lolvl}}
	= \diff\atlvl{\lolvl} \sumrate\atlvl{\lolvl-1}
	= \diff\atlvl{\lolvl} \parens{\rate\atlvl{0} + \dotsb + \rate\atlvl{\lolvl-1}}
\end{equation}
for all $\lvlalt=1,\dotsc,\nLvls-1$.
Thus, substituting \eqref{eq:sumweight} and \eqref{eq:weightrate} back into \eqref{eq:dKL-4}, we finally obtain
\begin{equation}
\label{eq:dKL-5}
\frac{d}{dt} \breg_{\nLvls}(\base,\orbit{\time})
	= \braket{\payv(\strat)}{\base}_{0} - \braket{\payv(\strat)}{\base}_{\nLvls}.
%	= \braket{\payv(\orbit{\time})}{\orbit{\time} - \base},
\end{equation}
However, since the only $0$-th level similarity class is $\pures$ itself (and $\base_{\pures} = 1$), we readily get
\begin{equation}
\braket{\payv(\strat)}{\base}_{0}
	= \base_{\pures} \; \classpay_{\pures}(\strat)
	= \sum_{\pure\in\pures} \strat_{\pure} \payv_{\pure}(\strat)
	= \braket{\payv(\strat)}{\strat}
\end{equation}
and our assertion follows.
\end{proof}


\cref{prop:KL} plays a crucial role in establishing the long-run rationality properties of \eqref{eq:NRD} recorded in \cref{thm:NRD}.
As an illustration, we sketch below the proof of the theorem's first item concerning the elimination of strictly dominated strategies.
For this, suppose that action $\pure\in\pures$ is strictly dominated by action $\purealt\in\pures$.
Then, if we let $\bvec_\pure\in \strats$ denote the ``pure'' population state corresponding to $\pure$ (and likewise for $\purealt$), the difference
\begin{equation}
\label{eq:TheBregDif}
\breg_{\nLvls}(\bvec_{\pure},\orbit{\time}) - \breg_{\nLvls}(\bvec_{\purealt},\orbit{\time})
	= \sum_{\lvl=1}^{\nLvls} \diff\atlvl{\lvl}
		\log\frac
			{\orbit[{\classof[\lvl]{\purealt}}]{\time}}
			{\orbit[{\classof[\lvl]{\pure}}]{\time}},
\end{equation}
is a weighted sum of log ratios of the masses of agents using actions in classes containing $\pure$ and $\purealt$.
It then follows from \cref{prop:KL} that
\begin{align}
\frac{d}{dt} \left(\vphantom{I^I}\breg_{\nLvls}(\bvec_{\pure},\orbit{\time}) - \breg_{\nLvls}(\bvec_{\purealt},\orbit{\time})\right)
	&= \braket{\payv(\orbit{\time})}{\orbit{\time} - \bvec_{\pure}} - \braket{\payv(\orbit{\time})}{\orbit{\time} - \bvec_{\purealt}}\notag\\
	%= \braket{\payv(\orbit{\time})}{\bvec_{\purealt} - \bvec_{\pure}}
	&= \payv_{\purealt}(\orbit{\time}) - \payv_{\pure}(\orbit{\time}).
	\label{eq:ThePayoffDiff}
\end{align}
Since $\purealt$ strictly dominates $\pure$, the payoff difference \eqref{eq:ThePayoffDiff} is positive and bounded away from zero.
Because of this, the difference \eqref{eq:TheBregDif} must grow without bound, which in turn implies that the population share $\strat_\pure$ of the dominated strategy $\pure$ vanishes.

For a detailed proof of the above claims and the remaining parts of \cref{thm:NRD}, we refer the reader to \cref{app:NRD}.

==> Body/Single.tex <==
%----------------------------------------------------------------------
%%% SINGLE
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


We now turn to our paper's main objective, the study of evolutionary dynamics in the presence of exogenous similarities and affinities between different actions in the population.
Specifically, as we discussed in the introduction, we aim to answer the following question:
\smallskip
\begin{quote}
\centering
\itshape
How are the dynamics affected if players take into account\\
similarities between strategies when revising them?
%How are the dynamics affected if players are more likely\\
%to imitate strategies that are similar to their own?
\end{quote}
\smallskip
For example,
a commuter may be more likely to switch to a different instance of their current transport mode, instead of a different transport mode altogether \citep[\eg taking a different combination of metro lines in Paris rather than switching to a bus line, \cf][]{BA73,BAL85,McF81,McF01}.
In a similar fashion,
when deciding to replace a computer or another consumer technology with network externalities, a consumer may be more likely to consider models manufactured by the maker of their current machine than those of other manufacturers, particularly in contexts with switching costs \citep{KS94,FarKle07}.
%a defensive chess player may be more likely to adopt winning endgame strategies of other defensive players rather than attacking players;
%etc.
%trees growing in the woods developing long straight trunks, with branching crowns high in the canopy, while the same species growing alone in the open develops a spreading form, branching much lower to the ground.

Our goal in this section is to provide a relatively simple framework for treating this question in a formal way;
the full model is subsequently presented in detail in \cref{sec:multiple}.



%----------------------------------------------------------------------
%%% Imitation under affinity
%----------------------------------------------------------------------
\subsection{Similarity-based imitation}
\label{sec:PPI-2}

Building on the \ac{PPI} protocol described in the previous section, we introduce below a more general family of revision protocols under which agents give additional consideration to switches to ``similar'' actions.
Formally, suppose that the set of alternatives $\pures$ comes equipped with a \emph{similarity partition} of the form
%$\classes = \{\class_{\iClass}\}_{\iClass=1}^{\nClasses}$
\begin{equation}
\label{eq:classes-single}
\classes = \setdef{\class_{\iClass} \subseteq \pures}{\iClass = 1,\dotsc,\nClasses}
\end{equation}
where the constituent \emph{similarity classes} $\class_{\iClass}$, $\iClass=1,\dotsc,\nClasses$,
are such that
$\union_{\iClass} \class_{\iClass} = \pures$
and
$\class_{\iClass} \cap \class_{\jClass} = \varnothing$ for all $\iClass \neq \jClass$
(\ie the similarity classes of $\classes$ cover $\pures$ and are mutually disjoint).
%(the meaning of the index ``$1$'' in $\classes$ will become clear later).
This partition of $\pures$ induces an equivalence relation ``$\sibling$'' on $\pures$, which we read as ``is similar to'', and which is defined in the obvious way:
$\pure\sibling\purealt$ if and only if $\pure,\purealt\in\class$ for some $\class\in\classes$.
In this way, each class $\class\in\classes$ represents a set of actions that share an exogenous similarity trait, which we assume that agents tend to respect when they revise (for example, instances of the same transport mode, computer models from the same manufacturer, etc.).
\smallskip

With all this in hand, we will consider the following similarity-aware revision process:
\begin{enumerate}
\item
When given the opportunity to switch strategies, the revising agent first decides whether to consider only the pool of similar strategies, or the entire population with no regard for similarities.
The first scenario occurs with probability $\rate\geq0$ (or, equivalently, for a fraction $\rate$ of the revising agents), the latter with probability $1 - \rate$.
\item
Conditioned on the above, the revising agent meets another individual \textendash\ the ``comparator'' \textendash\  uniformly at random.
Thus, if the population is at state $\strat\in\strats$, the probability that a revising $\pure$-strategist encounters a $\purealt$-strategist is
\begin{equation}
\label{eq:meet-single}
\pdist_{\pure\purealt}^{\textup{meet}}
	= \rate \, \strat_{\purealt \given \classof{\pure}}
		+ (1 - \rate) \, \strat_{\purealt}
\end{equation}
where
\begin{equation}
\label{eq:classof}
\classof{\pure}
%	= \setdef{\class\in\classes}{\class\ni\pure}
	= \setdef{\alt\pure\in\pures}{\alt\pure\sibling\pure}
\end{equation}
denotes the similarity class of $\pure$ in $\classes$ (that is, the set of strategies of $\pures$ that are similar to $\pure$) while, as per \eqref{eq:strat-cond}, the notation
\begin{equation}
\label{eq:strat-cond-2}
\strat_{\purealt \given \classof{\pure}}
	= \strat_{\purealt} \frac{\oneof{\purealt \in \classof{\pure}}}{\strat_{\classof{\pure}}}
\end{equation}
is shorthand for the relative frequency of $\purealt$-strategists within the sub-population of $\classof{\pure}$-type strategists (\ie the part of the population playing a strategy similar to $\pure$).
\item
As in the case of the standard \ac{PPI} protocol, the revising agent observes the comparator's payoff.
If the comparator has a higher payoff, the revising agent imitates their strategy with probability proportional to the observed payoff excess;
otherwise, the revising agent skips the opportunity to switch.
\end{enumerate}

Concretely, this process yields the \acli{SPPI} protocol
\begin{equation}
\label{eq:PPI-2}
\tag{PPI$_{2}$}
\switch_{\pure\purealt}(\py,\strat)
	= \rate \, \strat_{\purealt \given \classof{\pure}} \pospart{\py_{\purealt} - \py_{\pure}}
	+ (1 - \rate) \, \strat_{\purealt} \pospart{\py_{\purealt} - \py_{\pure}}
%	= 1-\rate \, \strat_{\purealt} \pospart{\py_{\purealt} - \py_{\pure}}
%	+ \rate \, \strat_{\purealt \given \classof{\pure}} \pospart{\py_{\purealt} - \py_{\pure}}
\end{equation}
where, as before, $\py \in \R^{\nPures}$ denotes the vector of payoffs in the population.%
\footnote{Since the conditional switch rate from an unused action is irrelevant \textendash\ in particular, it plays no role in \eqref{eq:MD} \textendash\ we define $\switch_{\pure\purealt}(\py,\strat)$ arbitrarily when $\strat_\pure = 0$.}
%\footnote{Here and throughout, we employ the useful notational convention that $\strat_{\purealt}/\strat_{\class} = 1/\abs{\class}$ if $\purealt\in\class$ and $\strat_{\class} = 0$ (so $\strat_{\purealt}=0$ by default).} 
In effect, unfolding this definition, a population of agents adhering to \eqref{eq:PPI-2} is running two pairwise comparison procedures at the same time:
\begin{enumerate}
\item
\emph{Intra-class revisions:}
Under the first procedure, which runs at rate $\rate$, the agent only considers switching to actions in the same similarity class as their current action.%
\footnote{For instance, the agent may observe randomly chosen opponents until encountering one who plays an action in $\classof{\pure}$.}
The agent then switches to action $\purealt \in \classof{\pure}$ only if their payoff is higher than that of $\pure$, and this with probability proportional to the payoff difference $\pospart{\py_{\purealt} - \py_{\pure}}$.
\item
\emph{Inter-class revisions:}
Under the second revision process, which runs at rate $1 - \rate$, the agent may consider switching to \emph{any} alternative action, irrespective of exogenous similarities.
Subsequently, as in the case of \eqref{eq:PPI}, switches occur at a rate proportional to the payoff difference $\pospart{\py_{\purealt} - \py_{\pure}}$.
\end{enumerate}

\begin{remark*}
The index ``$2$'' in \eqref{eq:PPI-2} and later in this section is meant to signify that similarities are examined relative to two different levels of $\pures$:
the partition into elements of $\classes$ and the partition into singletons (the finest possible partition).
In the next section, we will consider more general partition schemes with $\nLvls>2$ levels of exogenous similarities.
\endenv
\end{remark*}

An important feature of \eqref{eq:PPI-2} is that, ceteris paribus, imitation rates are always higher between similar strategies compared to dissimilar strategies \textendash\ \ie those that belong to the same class $\class$ of $\classes$ versus those that do not.
Indeed, in view of \eqref{eq:strat-cond-2}, the conditional switch rates $\switch_{\pure\purealt}$ of \eqref{eq:PPI-2} can be refactored as $\switch_{\pure\purealt}(\py,\strat) = \strat_{\purealt} \imit_{\pure\purealt}(\strat)$, where the conditional imitation rate $\imit_{\pure\purealt}(\strat)$, $\pure,\purealt\in\pures$, are given by
\begin{align}
\label{eq:imit-2}
\imit_{\pure\purealt}(\py,\strat)
%	= \parens*{1 - \rate + \rate \frac{\oneof{\purealt\in\classof{\pure}}}{\strat_{\classof{\pure}}}}
%		\pospart{\py_{\purealt} - \py_{\pure}}.
	&= \bracks*{1 + \rate \parens*{\frac{\oneof{\pure\sibling\purealt}}{\strat_{\classof{\pure}}} - 1}}
		\cdot \pospart{\py_{\purealt} - \py_{\pure}}
	\notag\\
	&= \pospart{\py_{\purealt} - \py_{\pure}}
		\cdot
		\begin{cases*}
			1 - \rate
				&\quad
				if $\pure\not\sibling\purealt$,
				\\
			1 - \rate + \rate/\strat_{\classof{\pure}}
				&\quad
				if $\pure\sibling\purealt$.
		\end{cases*}
\end{align}
Consequently,
for a given value of the payoff differential $\pospart{\py_{\purealt} - \py_{\pure}}$,
%if two strategies $\pure,\purealt\in\pures$ have the same payoff differential, say $\pospart{\py_{\purealt} - \py_{\pure}} = 1$,
the imitation rate of $\purealt$-strategists by $\pure$-strategists is higher if $\pure$ and $\purealt$ are similar compared to if they are not.

Importantly, this increased affinity toward similar strategies is an \emph{intrinsic} feature of the revision mechanism \eqref{eq:PPI-2}, and is due to the fact that a revising agent is more likely to meet another agent if the other agent's strategy is similar to their own \textendash\ more precisely, they have a higher conditional probability of encountering an individual from the sub-population of agents playing similar strategies.
This is reflected in the (state-dependent) factor $\extra_{\pure\purealt}(\strat) = \parens{1 -\rate} + \rate\cdot \oneof{\purealt\sibling\pure} / \strat_{\classof{\pure}}$ which adjusts upward the imitation rate from $\pure$ to $\purealt$ under \eqref{eq:PPI-2}:
since $\extra_{\pure\purealt}(\strat) \geq 1$,
%which indicates that the conditional imitation rate for a given strategy is proportional to its payoff difference (if positive) from the incumbent.
%Since $\strat_{\classof{\pure}} \leq 1$,
a direct comparison of the conditional imitation rates \eqref{eq:imit-1} and \eqref{eq:imit-2} \textendash\ for \eqref{eq:PPI} and \eqref{eq:PPI-2} respectively \textendash\ readily shows that
similar strategies are indeed imitated at a higher rate under \eqref{eq:PPI-2} compared to \eqref{eq:PPI}.
%In other words, the advantage provided by \eqref{eq:PPI-2} to similar strategies does not only extend to dissimilar strategies under \eqref{eq:PPI-2}, but also to similar strategies under the non-nested protocol \eqref{eq:PPI}.
\footnote{Of course, the inverse is true for dissimilar strategies, which are imitated at a lower rate under \eqref{eq:PPI-2} relative to \eqref{eq:PPI}.
Moreover, since the factor $\extra_{\pure\purealt}(\strat)$ increases as $\strat_{\classof{\pure}}\to0$, we also conclude that similarity classes that are less frequent in the population exhibit proportionally higher conditional switch rates.
%than they would otherwise get under the ordinary \ac{PPI} protocol.
By this token, \eqref{eq:PPI-2} provides a more level playing field and gives less of an advantage to strategies that are in abundance in a given state.}

The above should be contrasted to the scenario where an agent is equally likely to consider the actions of any other individual in the population, but is more likely to \emph{imitate} the strategy of the agent they meet if their strategies are more similar.%
\footnote{We are grateful to Tilman Börgers for this remark.}
In the simplest case, this scenario can be expressed as a revision protocol with conditional imitation rates given by
\begin{equation}
\label{eq:imit-2-alt}
\imit_{\pure\purealt}(\py,\strat)
	= \bracks*{\extra_{0} + \extra_{1} \, \oneof{\pure\sibling\purealt}}
		\cdot \pospart{\py_{\purealt} - \py_{\pure}}
\end{equation}
where $\extra_{0}$ is the base imitation rate,
while $\extra_{1} > 0$ measures the agents' additional drive toward imitating similar strategies.
Put differently, conditioned on an $\pure$-strategist encountering a $\purealt$-strategist when the population is at state $\strat\in\strats$ (an event that occurs with probability $\strat_{\pure}\strat_{\purealt}$), the conditional probability that the $\pure$-strategist \emph{imitates} the $\purealt$-strategist is now given by
%given that such an encounter occurred when the population is at state $\strat\in\strats$
%given that a revising $\pure$-strategist encountered a $\purealt$-strategist, the probability of imitation is given by
\begin{equation}
\pdist_{\pure\purealt}^{\textup{imit}}
	\propto \pospart{\py_{\purealt} - \py_{\pure}}
	 \cdot
	 \begin{cases*}
		\extra_{0}
			&\quad
			if $\pure \not\sibling \purealt$,
			\\
		\extra_{0} + \extra_{1}
			&\quad
			if $\pure\sibling\purealt$.
	\end{cases*}
\end{equation}
Under this protocol, similar strategies are favored \emph{extrinsically}:
they exhibit a higher conditional imitation rate relative to dissimilar ones but, otherwise, they are not encountered more often.
We discuss the evolutionary dynamics that result from this variant of \eqref{eq:PPI-2} in \cref{sec:discussion}.

%Finally, it is also worth comparing the agents' conditional imitation rates under \eqref{eq:PPI-2} to the homologous imitation rates under the \emph{non-nested} revision protocol \eqref{eq:PPI}, \viz
%\begin{equation}
%\label{eq:imit-1}
%\imit_{\pure\purealt}(\py,\strat)
%	= \pospart{\py_{\purealt} - \py_{\pure}}.
%\end{equation}
%%which indicates that the conditional imitation rate for a given strategy is proportional to its payoff difference (if positive) from the incumbent.
%Since $\strat_{\classof{\pure}} \leq 1$, a direct comparison of the imitation rates \eqref{eq:imit-2} and \eqref{eq:imit-1} readily yields that similar strategies are encountered and imitated at a higher rate under \eqref{eq:PPI-2} compared to \eqref{eq:PPI}.
%[And, of course, the inverse is true for dissimilar strategies, which are imitated at a lower rate under \eqref{eq:PPI-2} relative to \eqref{eq:PPI}.]
%In other words, the advantage provided by \eqref{eq:PPI-2} to similar strategies does not only extend to dissimilar strategies under \eqref{eq:PPI-2}, but also to similar strategies under the non-nested protocol \eqref{eq:PPI}.

%A different (but otherwise equivalent) interpretation of the similarity-based protocol \eqref{eq:PPI-2} can be obtained by using \eqref{eq:strat-cond} to rewrite the conditional selection probability $\strat_{\purealt\given\classof{\pure}}$ as
%\begin{equation}
%\label{eq:strat-cond-2}
%\strat_{\purealt\given\classof{\pure}}
%	= \strat_{\purealt} \cdot \oneof{\purealt \in \classof{\pure}} / \strat_{\classof{\pure}}
%\end{equation}
%where we used the straightforward identity $\strat_{\{\pure\} \cap \class} = \strat_{\pure} \oneof{\pure\in\class}$.
%The protocol \eqref{eq:PPI-2} may then be refactored as $\switch_{\pure\purealt}(\py,\strat) = \strat_{\purealt} \imit_{\pure\purealt}(\strat)$ with conditional imitation rates given by
%\begin{equation}
%\label{eq:imit-2}
%\imit_{\pure\purealt}(\py,\strat)
%	= \parens*{1 - \rate + \rate \frac{\oneof{\purealt\in\classof{\pure}}}{\strat_{\classof{\pure}}}}
%		\pospart{\py_{\purealt} - \py_{\pure}}
%\end{equation}
%for all $\pure,\purealt\in\pures$ and all $\strat\in\strats$, $\py\in\R^{\pures}$.
%In this regard, \eqref{eq:PPI-2} can be seen as a ``variable-rate'' version of \eqref{eq:PPI} in which revisions from $\purealt$ to $\pure$ are modulated by the (state-dependent) factor $\rate_{\pure\purealt}(\strat) = 1 - \rate + \rate\oneof{\purealt\in\classof{\pure}} / \strat_{\classof{\pure}}$.
%Since this factor increases as $\strat_{\classof{\pure}}\to0$, we conclude that, mutatis mutandis, similarity classes that are less frequent in the population get proportionally higher conditional switch rates than they would have under the ordinary \ac{PPI} protocol.
%By this token, \eqref{eq:PPI-2} provides a more level playing field and gives less of an advantage to strategies that are in abundance in a given population state.
%This point will become important in the sequel and we will return to it as needed.


%----------------------------------------------------------------------
%%% NRD-single
%----------------------------------------------------------------------
\subsection{The \acl{NRD}}
\label{sec:NRD-single}

We are now in a position to derive the evolution of the population's state under the nested protocol \eqref{eq:PPI-2}.
To that end, substituting \eqref{eq:PPI-2} into \eqref{eq:MD} readily yields
\begin{align}
\dot\strat_{\pure}
	&= (1-\rate)\, \strat_{\pure}
		\bracks*{
		\sum_{\purealt\in\pures} \strat_{\purealt} \pospart{\payv_{\pure}(\strat) - \payv_{\purealt}(\strat)}
		- \sum_{\purealt\in\pures} \strat_{\purealt} \pospart{\payv_{\purealt}(\strat) - \payv_{\pure}(\strat)}}
	\notag\\
	&+ \rate \strat_{\pure}
		\bracks*{
		\sum_{\purealt\in\classof{\pure}} \strat_{\purealt\given\classof{\pure}} \pospart{\payv_{\pure}(\strat) - \payv_{\purealt}(\strat)}
		- \sum_{\purealt\in\classof{\pure}} \strat_{\purealt\given\classof{\pure}} \pospart{\payv_{\purealt}(\strat) - \payv_{\pure}(\strat)}}.
\end{align}
and hence, after a slight rearrangement
\begin{equation}
\dot\strat_{\pure}
	= \strat_{\pure}
		\bracks*{%
		(1-\rate)\,
			\parens*{\payv_{\pure}(\strat) - \sum_{\purealt\in\pures} \strat_{\purealt} \payv_{\purealt}(\strat)}
		+ \rate
			\parens*{\payv_{\pure}(\strat) - \sum_{\purealt\in\classof{\pure}} \strat_{\purealt \given \classof{\pure}} \payv_{\purealt}(\strat)}
		} % end bracks
\end{equation}
Thus, rewriting the above in more compact form, we obtain the \acli{2RD}
\begin{equation}
\label{eq:NRD-single}
\tag{RD$_{2}$}
\dot\strat_{\pure}
	= (1-\rate)\,\,
		\strat_{\pure}
		\bracks{\payv_{\pure}(\strat) - \classpay_{\pures}(\strat)}
	+ \rate\,
		\strat_{\pure}
		\bracks{\payv_{\pure}(\strat) - \classpay_{\classof{\pure}}(\strat)}
\end{equation}
where
\begin{equation}
\label{eq:pay-class}
\classpay_{\class}(\strat)
	= \sum_{\pure\in\class} \strat_{\pure \given \class} \payv_{\pure}(\strat)
	= \frac{1}{\strat_{\class}} \sum_{\pure\in\class} \strat_{\pure} \payv_{\pure}(\strat)
\end{equation}
denotes the mean payoff of all actions in a subset $\class$ of $\pures$ (so, in particular, $\classpay_{\pures}(\strat) = \pay(\strat)$ by definition).
These dynamics are at the heart of our analysis, so some remarks are in order.

\setcounter{remark}{0}

\begin{remark}
The precise form of \eqref{eq:NRD-single} provides an interesting \textendash\ and informative \textendash\  interpretation of how population shares evolve under \eqref{eq:PPI-2}.
Specifically, the per capita growth rate of a strategy $\pure\in\pures$ under \eqref{eq:NRD-single} is a convex combination of two distinct payoff differences, with weights $1-\rate$ and $\rate$ respectively:
\begin{enumerate*}
[(\itshape i\hspace*{1pt}\upshape)]
\item
the difference between $\payv_{\pure}(\strat)$ and the \emph{aggregate} population mean $\classpay_{\pures}(\strat) = \pay(\strat)$ which is taken over \emph{all} strategies (irrespective of similarities);
and
\item
the difference between $\payv_{\pure}(\strat)$ and the \emph{cognate} population mean $\classpay_{\classof{\pure}}(\strat)$, which is taken over all \emph{similar} strategies.
\end{enumerate*}
Obviously, when $\rate= 0$, exogenous similarities between strategies are disregarded and \eqref{eq:NRD-single} reduces to the standard \acl{RD} \eqref{eq:RD}.
%, meaning that revising agents look at all actions simultaneously, oblivious to any exogenous similarities between them.
At the other end of the spectrum, when $\rate=1$, agents only look within their class and never switch to dissimilar actions.
To avoid complicating the presentation, we exclude this extreme case below, requiring instead that the full set of actions be contemplated at a positive rate.
\endenv
\end{remark}

\begin{remark}
Importantly, if we sum \eqref{eq:NRD-single} over all actions belonging to the same similarity class $\class\in\classes$, the second term in \eqref{eq:NRD-single} vanishes and the first takes the simple form
\begin{equation}
\label{eq:NRD-single-class}
\dot\strat_{\class}
	= \sum_{\pure\in\class} \dot\strat_{\pure}
	= (1-\rate)\,
		\strat_{\class}\,
		\bracks*{\classpay_{\class}(\strat) - \classpay_{\pures}(\strat)},
\end{equation}
According to \eqref{eq:NRD-single-class}, the evolution of the population share $\strat_{\class}$ of each class $\class\in\classes$ is governed by a formal analogue of the \acl{RD} \eqref{eq:RD} rescaled by a factor of $1-\rate$ (that is, the agents' inter-class revision rate).
The main difference between \eqref{eq:NRD-single-class} and a replicator system evolving on the simplex $\simplex(\classes)$ is that the class-averaged payoffs $\classpay_{\class}(\strat)$ in \eqref{eq:NRD-single-class} do not depend only on the various class frequencies $\strat_{\class}$, $\class\in\classes$, but on the \emph{complete} $\nElems$-dimensional population state $\strat\in\simplex(\pures)$.
On that account, the dynamics \eqref{eq:NRD-single} provide much finer information than the aggregate system \eqref{eq:NRD-single-class}, so the latter cannot be used as an autonomous surrogate for the former.
%\footnote{For instance, note that different values of the ``global'' revision rate $1-\rate$ are not reflected in \eqref{eq:NRD-single-class}.}
\endenv
\end{remark}

\begin{remark}
One last point worth noting is a crucial difference between the nested dynamics \eqref{eq:NRD-single} and their non-nested counterpart \eqref{eq:RD}.
Specifically, the per capita growth rate $\growth_{\pure}(\strat) = \dot\strat_{\pure}/\strat_{\pure}$ of strategy $\pure\in\pures$ under \eqref{eq:NRD-single} can be written as
\begin{equation}
\label{eq:grow-2}
\growth_{\pure}(\strat)
	= \payv_{\pure}(\strat)
		- (1-\rate)\,\, \classpay_{\pures}(\strat)
		- \rate\, \classpay_{\classof{\pure}}(\strat)
\end{equation}
so, for any pair of strategies $\pure,\purealt\in\pures$, we have
\begin{equation}
\label{eq:growdiff-2}
\growth_{\pure}(\strat) - \growth_{\purealt}(\strat)
	= \payv_{\pure}(\strat) - \payv_{\purealt}(\strat)
		- \rate\, \bracks{\classpay_{\classof{\pure}}(\strat) - \classpay_{\classof{\purealt}}(\strat)}.
\end{equation}
Clearly, if $\pure$ and $\purealt$ belong to the same similarity class of $\classes$, \eqref{eq:growdiff-2} gives $\growth_{\pure}(\strat) - \growth_{\purealt}(\strat) = \payv_{\pure}(\strat) - \payv_{\purealt}(\strat)$, so the dynamics \eqref{eq:NRD-single} exhibit payoff-monotone growth rates within the \emph{same} similarity class.%
\footnote{Following \citet{San10,San15} and \citet{Wei95}, payoff monotonicity means here that $\growth_{\pure}(\strat) \geq \growth_{\purealt}(\strat)$ if and only if $\payv_{\pure}(\strat) \geq \payv_{\purealt}(\strat)$.}
On the other hand, if $\pure$ and $\purealt$ belong to different similarity classes, the difference $\classpay_{\classof{\pure}}(\strat) - \classpay_{\classof{\purealt}}(\strat)$ could be arbitrarily large relative to $\payv_{\pure}(\strat) - \payv_{\purealt}(\strat)$ and with a different sign.
Thus, in stark contrast to the standard \acl{RD} \eqref{eq:RD}, the nested dynamics \eqref{eq:NRD-single} \emph{are not payoff-monotonic}, a fact which poses significant obstacles to their analysis.
We will return to this point in the sequel.%
\footnote{In view of \eqref{eq:imit-2}, \citet{Wei95} would call \eqref{eq:PPI-2} an ``imitative'' protocol.
This clashes with the terminology of \citet[Chap.~5.4]{San10}, where an additional payoff monotonicity condition is required;
as we discussed above, the monotonicity requirement of \citet{San10} \emph{fails} for \eqref{eq:PPI-2}, so we do not use the term ``imitative'' to avoid ambiguity.
For a detailed discussion on the differences between ``imitative'' and ``monotone imitative'' dynamics, see \citet{MV22}.}

\end{remark}

%----------------------------------------------------------------------
%%% First results
%----------------------------------------------------------------------
\subsection{Rationality properties}
\label{sec:results-2}

%\WHS{Below I put ``strictly'' back in front of ``dominated''. Economists will expect this distinction to be made.}

The \acl{RD} have been studied extensively in the literature, and their stability and convergence properties are a staple of evolutionary game theory.
Following \citet{HS88}, \citet{Wei95} and \citet{San10}, their most important properties can be summarized as follows:
\begin{enumerate}
%\setlength{\itemsep}{.5ex}
\item
Strictly dominated actions become extinct.
\item
All \aclp{NE} are stationary, and all locally stable states are Nash equilibria;
neither converse statement holds.
\item
Evolutionarily stable states are locally attracting.
\item
Interior solutions converge to \acl{NE} in generic potential and strictly contractive games.
\end{enumerate}

Stating these properties formally requires a number of standard definitions from the theory of dynamical systems.
To maintain the flow of our discussion, we relegate these definitions (along with some technical details) to \cref{app:defs},
and we proceed below to state the main long-run rationality properties of the two-level dynamics \eqref{eq:NRD-single}:
%and we refer the reader to \citet{Wei95} and \citet{San10} for further examples and discussions.


\begin{theorem}
\label{thm:NRD-single}
Let $\game\equiv\gamefull$ be a population game and let $\orbit{\time}$ be an interior solution trajectory of the \acl{NRD} \eqref{eq:NRD-single} for $\game$.
We then have:
\begin{enumerate}
[1.]
%[\upshape(\itshape i\hspace*{1pt}\upshape)]
%\setlength{\itemsep}{.5ex}
\item
If $\pure \in \pures$ is strictly dominated, then $\lim_{\time\to\infty} \orbit[\pure]{\time} = 0$.

\item
A state $\eq\in\strats$ is stationary if and only if it is a \acl{RE} of $\game$.

\item
\label{itm:ImpliesNE}
If $\orbit{\time}$ converges to $\eq$ as $\time\to\infty$, then $\eq$ is a \acl{NE} of $\game$.

\item
\label{itm:ImpliesNE}
If $\eq\in\strats$ is Lyapunov stable, then it is a \acl{NE} of $\game$.

\item
If $\eq$ is an \ac{ESS} of $\game$, it is asymptotically stable. %\textpar{so it attracts all nearby initial conditions $x(0)\in\strats$}.
In particular, if $\eq$ is a \ac{GESS} of $\game$, it attracts all initial conditions with $\supp(\strat(\tstart)) \supseteq \supp(\eq)$.

\item
If $\game$ is a potential game with potential function $\pot$, then $\pot(\orbit{\time})$ is nondecreasing and $\orbit{\time}$ converges to a connected set of restricted equilibria of $\game$.

\item
If $\game$ is strictly monotone, its \textpar{necessarily unique} \acl{NE} attracts almost all initial conditions \textendash\ and, in particular, all initial conditions with full support.
\end{enumerate}
\end{theorem}

\cref{thm:NRD-single} is a special case of the more general \cref{thm:NRD}, which we present and discuss in detail in \cref{sec:multiple}.
Of course, when agents do not consider intra-group similarities ($\rate=0$), we recover known properties of the \acl{RD} \eqref{eq:RD}.
However, in contrast to the non-nested case, the dynamics \eqref{eq:NRD-single} are \emph{not} payoff-monotone, so there seems to be no particular reason to expect that the above properties should continue to hold in the nested case as well.

To gain some intuition in the proof of \cref{thm:NRD-single},
%with the work of \citet{HSS79} (see also \citealp{HS88} and \citealp{Wei95}),
a key observation is that the properties mentioned above for \eqref{eq:RD} are closely linked to the so-called \acdef{KL} \emph{divergence}, defined for each base point $\base\in\strats$ and test state $\strat\in\strats$ as
\begin{equation}
\label{eq:KL}
\tag{KL}
\breg(\base,\strat)
	= \sum_{\pure\in\pures} \base_{\pure} \log\frac{\base_{\pure}}{\strat _{\pure}}.
\end{equation}
By definition, this asymmetric measure of ``distance'' between $\base$ and $\strat$
is nonnegative,
it becomes infinite only when $\supp(\base)\nsubseteq\supp(\strat)$,
and
vanishes if and only if $\strat=\base$.
Through these properties, as well as others linking it directly to the \acl{RD} (\cf~\cref{prop:KL} later), the \ac{KL} divergence provides a natural device for examining the long-run evolution of the trajectories of \eqref{eq:RD} relative to the base point $\base\in\strats$.
%to check both divergence from and convergence to a base point $\base\in\strats$.

For the nested dynamics \eqref{eq:NRD-single}, the mixing of intra- and inter-class comparisons complicates things considerably, and the \ac{KL} divergence is no longer a relevant measure of distance.
Instead, with the benefit of hindsight, we need to consider the (\emph{two-level}) \emph{nested} \acl{KL} divergence
\begin{equation}
\label{eq:KL-2}
\tag{KL$_{2}$}
\breg_{2}(\base,\strat )
%	= \frac{1}{1-\rate + \rate}
%		\bracks*{
	= \sum_{\pure\in\pures} \base_{\pure} \log\frac{\base_{\pure}}{\strat_{\pure}}
		+ \frac{\rate}{1-\rate}
		\sum_{\class\in\classes} \base_{\class} \log\frac{\base_{\class}}{\strat_{\class}}
%		}.
%		\sum_{\pure\in\supp(\base)} \base_{\pure}
%		\bracks*{\log\frac{\base_{\pure}}{\strat_{\pure}} + \frac{\rate}{1-\rate} \log\frac{\base_{\classof{\pure}}}{\strat_{\classof{\pure}}}}.
\end{equation}
The definition of $\breg_{2}$ is at the same time natural and somewhat sibylline:
on the one hand, it is natural to expect that any measure of distance attuned to \eqref{eq:NRD-single} would involve a mixing of action and class population shares ($\strat_{\pure}$ and $\strat_{\class}$ respectively);
on the other hand, the precise nature of the coefficients and the type of mixing cannot be guessed in advance (at least, not in any principled way), and it requires a fair amount of reverse engineering.
%\eqref{eq:KL-2} combines action and class population shares in a manner akin to \eqref{eq:NRD-single}.
The details of this derivation are presented and explained in \cref{app:NLC};
for now, we simply note that the case $\rate=0$, which yields the standard \acl{RD} \eqref{eq:RD}, also yields the standard \acl{KL} divergence \eqref{eq:KL}.
